Improving Federated Learning Communication Efficiency with Global Momentum Fusion for Gradient Compression Schemes

Communication costs within Federated learning hinder the system scalability for reaching more data from more clients. The proposed FL adopts a hub-and-spoke network topology. All clients communicate through the central server. Hence, reducing communication overheads via techniques such as data compression has been proposed to mitigate this issue. Another challenge of federated learning is unbalanced data distribution, data on each client are not independent and identically distributed (non-IID) in a typical federated learning setting. In this paper, we proposed a new compression compensation scheme called Global Momentum Fusion (GMF) which reduces communication overheads between FL clients and the server and maintains comparable model accuracy in the presence of non-IID data. GitHub repository: https://github.com/tony92151/global-momentum-fusion-fl

==> figure/task2_acc_cr01_.tex <==
\begin{figure}[htb]
\vspace{-1em}    
\centering  
\includegraphics[width=8cm]{pdf/mix_plots_0.1_acc.pdf}  
\vspace{-0.5em}   
\caption{Top-1 Accuracy curves on Shakespeare}  
\label{fig:task2_top1_accuracy}  
\vspace{-1.3em}  % 調整上下文間距
\end{figure}
